NeuFA: Neural Network Based End-to-End Forced Alignment with Bidirectional Attention Mechanism

Although deep learning and end-to-end models have been widely used and shown superiority in automatic speech recognition (ASR) and text-to-speech (TTS) synthesis, state-of-the-art forced alignment (FA) models are still based on hidden Markov model (HMM). HMM has limited view of contextual information and is developed with long pipelines, leading to error accumulation and unsatisfactory performance. Inspired by the capability of attention mechanism in capturing long term contextual information and learning alignments in ASR and TTS, we propose a neural network based end-to-end forced aligner called NeuFA, in which a novel bidirectional attention mechanism plays an essential role. NeuFA integrates the alignment learning of both ASR and TTS tasks in a unified framework by learning bidirectional alignment information from a shared attention matrix in the proposed bidirectional attention mechanism. Alignments are extracted from the learnt attention weights and optimized by the ASR, TTS and FA tasks in a multi-task learning manner. Experimental results demonstrate the effectiveness of our proposed model, with mean absolute error on test set drops from 25.8 ms to 23.7 ms at word level, and from 17.0 ms to 15.7 ms at phoneme level compared with state-of-the-art HMM based model.

==> content/abstract2.tex <==
\begin{abstract}
Although deep learning and end-to-end models have already applied and shown their superiority in
automatic speech recognition (ASR) and text-to-speech (TTS) synthesis,
state-of-the-art force alignment (FA) models are still based on the hidden Markov model (HMM).
%which only have limited views of contextual information.
%Moreover, 
Developing such long pipelines are not only
resource-consuming,
but also causing error compounding and unsatisfied results.
Moreover, only the ASR direction is used to learn alignments in these models,
neglecting the input texts and the TTS direction which is also known to be capable to learning alignments.
%and limited uses of the texts to be aligned since they are developed from ASR models.
%These lead to unsatisfied results in FA.
%than the end-to-end models used in ASR and TTS,
%Also the texts information are rarely considered when training these FA models 
To address these problems
and improve FA with deep learning and end-to-end technologies,
%and take full use of both the acoustic and textual information in inputs,
%and simply the development of FA models 
%in this paper,
we propose NeuFA, a neural network based end-to-end force aligner, 
and bidirectional attention mechanism which is the most essential algorithm used in NeuFA.
NeuFA utilizes both the ASR and TTS directions in a same training framework with the bidirectional attention mechanism.
The bidirectional attention mechanism provides shared attention matrices for both the ASR and TTS directions for each pair of inputs.
Then alignments can be extracted from the attention matrices and optimized by both directions in a multi-task learning manner.
%Then boundaries are extracted from these shared attention matrices at word and phoneme levels.
Experimental results the effectiveness of our proposed model,
with mean absolute error (MAE) of word boundaries dropped from 26 ms to 24 ms 
and MAE of phoneme boundaries dropped from 17 ms to 15 ms than state-of-the-art HMM based models,
%Then alignments are extracted from the 
%from which both the ASR and TTS tasks are con
%in which the input texts and speeches are trying to predict each other.
%And alignments are learnt though the shared attention matrices 
%in the proposed bidirectional attention mechanism
%used in both the ASR and TTS tasks
%for each pair of inputs.
\end{abstract}

==> content/figure.tex <==
\begin{figure*}[t]
	\centering
	\begin{minipage}[b]{0.465\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figure/neufa}
		(a) Neural network based FA with bidirectional attention
	\end{minipage}
	\hfill
	\begin{minipage}[b]{0.28\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figure/position.png}
		(b) Adding original and estimated positional encodings\\
		\text{}\\
		\includegraphics[width=.755\linewidth]{figure/diagonal.png}\\
		(c) Diagonal weight matrix in the diagonal attention loss
	\end{minipage}
	\hfill
	\begin{minipage}[b]{0.2225\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figure/attention1.png}
		(d) Attention weights for TTS
		\includegraphics[width=\linewidth]{figure/attention2.png}
		(e) Attention weights for ASR
		\includegraphics[width=\linewidth]{figure/attention3.png}
		(f) Predicted boundaries
		%\\\text{}\\
		%\includegraphics[width=\linewidth]{figures/tts.png}
		%(c) Conversational TTS framework
	\end{minipage}
	\caption{
	    (a) Architecture of NeuFA, the proposed neural network based force alignment model.
	    (b) Model architecture for adding original and estimated positional encodings.
	    (c) Illustration of an diagonal weight matrix used in the diagonal attention loss.
	    (d) Illustration of learnt attention weights for TTS.
	    (e) Illustration of learnt attention weights for ASR.
	    (f) Illustration of predicted (green) and ground-truth (yellow) phoneme boundaries.
	}
	\label{fig:structure}
\end{figure*}

==> content/figure2.tex <==
\begin{figure*}[t]
	\centering
	\begin{minipage}[b]{0.465\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figure/neufa.png}\\
		(a) Neural network based FA with bidirectional attention\\
		\includegraphics[height=2.5cm]{figure/attention2.png}\\
		(a) Neural network based FA with bidirectional attention
	\end{minipage}
	\hfill
	\begin{minipage}[b]{0.35\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figure/attention.png}\\
		(a) Neural network based FA with bidirectional attention\\
		\includegraphics[height=2.5cm]{figure/attention2.png}\\
		(a) Neural network based FA with bidirectional attention
	\end{minipage}
	\hfill
	\begin{minipage}[b]{0.15\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figure/position.pdf}\\
		(b) Illustration of adding original and estimated positional encodings\\
		\includegraphics[height=2.5cm]{figure/attention3.png}\\
		(c) An example of learnt attention weights for ASR and TTS
		%\\\text{}\\
		%\includegraphics[width=\linewidth]{figures/tts.png}
		%(c) Conversational TTS framework
	\end{minipage}
	\caption{
	    (a) Architecture of the proposed spoken style learning method with multi-model hierarchical context encoding. %for conversational TTS.
	    (b) Architecture of the speaker-independent global style token enhanced Tacotron framework.
	    (c) Architecture of the conversational TTS framework.
	}
	\label{fig:structure}
\end{figure*}

==> content/introduction2.tex <==
\section{Introduction}
With the development of deep learning and end-to-end technology,
many neural network based models are proposed for automatic speech recognition (ASR) \cite{chan_listen_2016, gulati_conformer_2020} 
and text-to-speech (TTS) synthesis \cite{wang_tacotron:_2017, shen_natural_2017, ren_fastspeech_2019, ren_fastspeech_2020} and outperform conventional methods.
%The attention mechanism has also shown its capability of learning alignments in these tasks and whether the alignments are learnt
These models are commonly developed in encoder-decoder with attention framework \cite{bahdanau_neural_2014},
from which the encoder and decoder convert the sequences between texts and speeches,
%in end-to-end manners and commonly employ 
and the attention mechanism \cite{vaswani_attention_2017} is employed to capture a long view of contextual information for current decoding step.

However, state-of-the-art forced alignment (FA) models are still based on the hidden Markov model (HMM) \cite{rabiner_introduction_1986} and developed with long pipelines.
%which only have limited views of contextual information.
%Moreover, 
HMM only has a limited view of contextual information.
And developing such long pipelines are not only
resource-consuming,
but also causing error compounding and leading to unsatisfied results.
%Moreover, these models are always developed from ASR models which neglects or doesn't take full use of the input texts information.
%These issues lead to unsatisfied results in FA.

The attention mechanism used in state-of-the-art ASR and TTS models 
has shown this capability of learning alignment information and improved model interpretability.
It is of possibility to build a neural network model for FA if the alignments can be extracted from the alignment information learnt by the attention mechanism.
Moreover, the alignment information can be learnt from both the ASR and TTS tasks.
And further improvement is also of possibility to be made if the alignments can be optimized by both tasks in a multi-task learning manner.

%only the ASR direction is used to learn alignments in these models,
%and the TTS direction which is also known to be capable to learning alignments.
%and limited uses of the texts to be aligned since they are developed from ASR models.
%These lead to unsatisfied results in FA.
%than the end-to-end models used in ASR and TTS,
%Also the texts information are rarely considered when training these FA models 

In this paper,
to improve FA with deep learning and end-to-end technologies,
%inspired by the attention mechanism \cite{} and its capability of learning alignment information,
we propose a neural network based end-to-end forced aligner which is called NeuFA,
and bidirectional attention mechanism which is the most essential algorithm used in NeuFA.
The bidirectional attention mechanism are extended from the original attention mechanism to learn bidirectional relation mapping between two sets of key-value pairs.
And NeuFA integrates the alignment learning of both the ASR and TTS tasks in a same training framework by learning bidirectional alignment information in the proposed the bidirectional attention mechanism.
The bidirectional alignment information is learnt by the shared attention matrix in bidirectional attention mechanism and optimized by both two tasks in a multi-task learning manner.
Then the attention weights for two tasks are obtained from the shared attention matrix
and converted to boundaries at word or phoneme level by a boundary detector.
%The bidirectional attention mechanism provides shared attention matrices for both the ASR and TTS directions for each pair of inputs.
%Then alignments can be extracted from the attention matrices and optimized by both directions in a multi-task learning manner.
%Then boundaries are extracted from these shared attention matrices at word and phoneme levels.
Experimental results demonstrate the effectiveness of our proposed model,
with mean absolute error (MAE) on test set drops from 25.8 ms to 23.7 ms at word level,
and drops from 17.0 ms to 15.7 ms at phoneme level
than state-of-the-art HMM based model.
The source code of NeuFA will be released on GitHub when the paper is accepted.
%The source code of NeuFA is available at https://github.com/thuhcsi/NeuFA.
%Then alignments are extracted from the 
%from which both the ASR and TTS tasks are con
%in which the input texts and speeches are trying to predict each other.
%And alignments are learnt though the shared attention matrices 
%in the proposed bidirectional attention mechanism
%used in both the ASR and TTS tasks
%for each pair of inputs.
